Resource-Scalable CNN Synthesis for IoT Applications

State-of-the-art image recognition systems use sophisticated Convolutional Neural Networks (CNNs) that are designed and trained to identify numerous object classes. Such networks are fairly resource intensive to compute, prohibiting their deployment on resource-constrained embedded platforms. On one hand, the ability to classify an exhaustive list of categories is excessive for the demands of most IoT applications. On the other hand, designing a new custom-designed CNN for each new IoT application is impractical, due to the inherent difficulty in developing competitive models and time-to-market pressure. To address this problem, we investigate the question of: "Can one utilize an existing optimized CNN model to automatically build a competitive CNN for an IoT application whose objects of interest are a fraction of categories that the original CNN was designed to classify, such that the resource requirement is proportionally scaled down?" We use the term resource scalability to refer to this concept, and develop a methodology for automated synthesis of resource scalable CNNs from an existing optimized baseline CNN. The synthesized CNN has sufficient learning capacity for handling the given IoT application requirements, and yields competitive accuracy. The proposed approach is fast, and unlike the presently common practice of CNN design, does not require iterative rounds of training trial and error.

==> arxiv <==
@inproceedings{iandola2017small,
	title={Small neural nets are beautiful: enabling embedded systems with small deep-neural-network architectures},
	author={Forrest et al.},
	booktitle={Proceedings of the Twelfth IEEE/ACM/IFIP International Conference on Hardware/Software Codesign and System Synthesis Companion},
	pages={1},
	year={2017},
	organization={ACM}
}
@article{verhelst2017embedded,
	title={Embedded Deep Neural Network Processing: Algorithmic and Processor Techniques Bring Deep Learning to IoT and Edge Devices},
	author={Verhelst, Marian and Moons, Bert},
	journal={IEEE Solid-State Circuits Magazine},
	volume={9},
	number={4},
	pages={55--65},
	year={2017},
	publisher={IEEE}
}
@article{iandola2016squeezenet,
	title={Squeezenet: Alexnet-level accuracy with 50x fewer parameters and< 0.5 mb model size},
	author={Iandola, Forrest N and Han, Song and Moskewicz, Matthew W and Ashraf, Khalid and Dally, William J and Keutzer, Kurt},
	journal={arXiv preprint arXiv:1602.07360},
	year={2016}
}
@article{DistillNet,
	title={Reference removed for blind review purposes}
}
@article{Octopus,
	title={Reference removed for blind review purposes}
}
@article{sze2017efficient,
	title={Efficient processing of deep neural networks: A tutorial and survey},
	author={Sze, Vivienne and Chen, Yu-Hsin and Yang, Tien-Ju and Emer, Joel S},
	journal={Proceedings of the IEEE},
	volume={105},
	number={12},
	pages={2295--2329},
	year={2017},
	publisher={IEEE}
}
@article{lin2018focal,
	title={Focal loss for dense object detection},
	author={Lin, Tsung-Yi and Goyal, Priyal and Girshick, Ross and He, Kaiming and Doll{\'a}r, Piotr},
	journal={IEEE transactions on pattern analysis and machine intelligence},
	year={2018},
	publisher={IEEE}
}
@inproceedings{deng2009imagenet,
  title={Imagenet: A large-scale hierarchical image database},
  author={Deng et al.},
  booktitle={Computer Vision and Pattern Recognition, IEEE Conference on},
  pages={248--255},
  year={2009},
  organization={IEEE}
}
@inproceedings{szegedy2015going,
	title={Going deeper with convolutions},
	author={Szegedy, Christian and Liu, Wei and Jia, Yangqing and Sermanet, Pierre and Reed, Scott and Anguelov, Dragomir and Erhan, Dumitru and Vanhoucke, Vincent and Rabinovich, Andrew and others},
	year={2015},
	organization={Cvpr}
}
@article{russakovsky2015imagenet,
	title={Imagenet large scale visual recognition challenge},
	author={Russakovsky et al.},
	journal={International Journal of Computer Vision},
	volume={115},
	number={3},
	pages={211--252},
	year={2015},
	publisher={Springer}
}
@inproceedings{krizhevsky2012imagenet,
	title={Imagenet classification with deep convolutional neural networks},
	author={Krizhevsky, Alex and Sutskever, Ilya and Hinton, Geoffrey E},
	booktitle={Advances in neural information processing systems},
	pages={1097--1105},
	year={2012}
}
@inproceedings{zhang2015optimizing,
	title={Optimizing fpga-based accelerator design for deep convolutional neural networks},
	author={Zhang, Chen and Li, Peng and Sun, Guangyu and Guan, Yijin and Xiao, Bingjun and Cong, Jason},
	booktitle={Proceedings of the 2015 ACM/SIGDA International Symposium on Field-Programmable Gate Arrays},
	pages={161--170},
	year={2015},
	organization={ACM}
}
@inproceedings{motamedi2016design,
	title={Design space exploration of fpga-based deep convolutional neural networks},
	author={Motamedi, Mohammad and Gysel, Philipp and Akella, Venkatesh and Ghiasi, Soheil},
	booktitle={Design Automation Conference (ASP-DAC), 2016 21st Asia and South Pacific},
	pages={575--580},
	year={2016},
	organization={IEEE}
}
@inproceedings{qiu2016going,
	title={Going deeper with embedded fpga platform for convolutional neural network},
	author={Qiu, Jiantao and Wang, Jie and Yao, Song and Guo, Kaiyuan and Li, Boxun and Zhou, Erjin and Yu, Jincheng and Tang, Tianqi and Xu, Ningyi and Song, Sen and others},
	booktitle={Proceedings of the 2016 ACM/SIGDA International Symposium on Field-Programmable Gate Arrays},
	pages={26--35},
	year={2016},
	organization={ACM}
}
@article{ovtcharov2015accelerating,
	title={Accelerating deep convolutional neural networks using specialized hardware},
	author={Ovtcharov, Kalin and Ruwase, Olatunji and Kim, Joo-Young and Fowers, Jeremy and Strauss, Karin and Chung, Eric S},
	journal={Microsoft Research Whitepaper},
	volume={2},
	number={11},
	year={2015}
}
@inproceedings{chen2014dadiannao,
	title={Dadiannao: A machine-learning supercomputer},
	author={Chen, Yunji and Luo, Tao and Liu, Shaoli and Zhang, Shijin and He, Liqiang and Wang, Jia and Li, Ling and Chen, Tianshi and Xu, Zhiwei and Sun, Ninghui and others},
	booktitle={Proceedings of the 47th Annual IEEE/ACM International Symposium on Microarchitecture},
	pages={609--622},
	year={2014},
	organization={IEEE Computer Society}
}
@article{shafiee2016isaac,
	title={ISAAC: A convolutional neural network accelerator with in-situ analog arithmetic in crossbars},
	author={Shafiee, Ali and Nag, Anirban and Muralimanohar, Naveen and Balasubramonian, Rajeev and Strachan, John Paul and Hu, Miao and Williams, R Stanley and Srikumar, Vivek},
	journal={ACM SIGARCH Computer Architecture News},
	volume={44},
	number={3},
	pages={14--26},
	year={2016},
	publisher={ACM}
}
@inproceedings{jouppi2017datacenter,
	title={In-datacenter performance analysis of a tensor processing unit},
	author={Jouppi, Norman P and Young, Cliff and Patil, Nishant and Patterson, David and Agrawal, Gaurav and Bajwa, Raminder and Bates, Sarah and Bhatia, Suresh and Boden, Nan and Borchers, Al and others},
	booktitle={Proceedings of the 44th Annual International Symposium on Computer Architecture},
	pages={1--12},
	year={2017},
	organization={ACM}
}
@article{motamedi2018cappuccino,
	title={Cappuccino: Efficient CNN Inference Software Synthesis for Mobile System-on-Chips},
	author={Motamedi, Mohammad and Fong, Daniel and Ghiasi, Soheil},
	journal={IEEE Embedded Systems Letters},
	year={2018},
	publisher={IEEE}
}
@article{gysel2016hardware,
	title={Hardware-oriented approximation of convolutional neural networks},
	author={Gysel, Philipp and Motamedi, Mohammad and Ghiasi, Soheil},
	journal={arXiv preprint arXiv:1604.03168},
	year={2016}
}
@article{iandola2016squeezenet,
	title={SqueezeNet: AlexNet-level accuracy with 50x fewer parameters and< 0.5 MB model size},
	author={Iandola, Forrest N and Han, Song and Moskewicz, Matthew W and Ashraf, Khalid and Dally, William J and Keutzer, Kurt},
	journal={arXiv preprint arXiv:1602.07360},
	year={2016}
}
@article{han2015deep,
	title={Deep compression: Compressing deep neural networks with pruning, trained quantization and huffman coding},
	author={Han et al.},
	journal={arXiv preprint arXiv:1510.00149},
	year={2015}
}
@inproceedings{hassibi1993optimal,
	title={Optimal brain surgeon and general network pruning},
	author={Hassibi, Babak and Stork, David G and Wolff, Gregory J},
	booktitle={Neural Networks, 1993., IEEE International Conference on},
	pages={293--299},
	year={1993},
	organization={IEEE}
}
@article{li2016pruning,
	title={Pruning filters for efficient convnets},
	author={Li, Hao and Kadav, Asim and Durdanovic, Igor and Samet, Hanan and Graf, Hans Peter},
	journal={arXiv preprint arXiv:1608.08710},
	year={2016}
}
@inproceedings{hubara2016binarized,
	title={Binarized neural networks},
	author={Hubara, Itay and Courbariaux, Matthieu and Soudry, Daniel and El-Yaniv, Ran and Bengio, Yoshua},
	booktitle={Advances in neural information processing systems},
	pages={4107--4115},
	year={2016}
}
@inproceedings{rastegari2016xnor,
	title={Xnor-net: Imagenet classification using binary convolutional neural networks},
	author={Rastegari, Mohammad and Ordonez, Vicente and Redmon, Joseph and Farhadi, Ali},
	booktitle={European Conference on Computer Vision},
	pages={525--542},
	year={2016},
	organization={Springer}
}
@inproceedings{alzantot2017rstensorflow,
	title={Rstensorflow: Gpu enabled tensorflow for deep learning on commodity android devices},
	author={Alzantot, Moustafa and Wang, Yingnan and Ren, Zhengshuang and Srivastava, Mani B},
	booktitle={Proceedings of the 1st International Workshop on Deep Learning for Mobile Systems and Applications},
	pages={7--12},
	year={2017},
	organization={ACM}
}
@inproceedings{han2015learning,
	title={Learning both weights and connections for efficient neural network},
	author={Han et al.},
	booktitle={Advances in neural information processing systems},
	pages={1135--1143},
	year={2015}
}
@inproceedings{han2016eie,
	title={EIE: efficient inference engine on compressed deep neural network},
	author={Han, Song and Liu, Xingyu and Mao, Huizi and Pu, Jing and Pedram, Ardavan and Horowitz, Mark A and Dally, William J},
	booktitle={Computer Architecture (ISCA), 2016 ACM/IEEE 43rd Annual International Symposium on},
	pages={243--254},
	year={2016},
	organization={IEEE}
}
@inproceedings{he2014reshaping,
	title={Reshaping deep neural network for fast decoding by node-pruning},
	author={He, Tianxing and Fan, Yuchen and Qian, Yanmin and Tan, Tian and Yu, Kai},
	booktitle={Acoustics, Speech and Signal Processing (ICASSP), 2014 IEEE International Conference on},
	pages={245--249},
	year={2014},
	organization={IEEE}
}
@article{motamedi2017machine,
	title={Machine Intelligence on Resource-Constrained IoT Devices: The Case of Thread Granularity Optimization for CNN Inference},
	author={Motamedi, Mohammad and Fong, Daniel and Ghiasi, Soheil},
	journal={ACM Transactions on Embedded Computing Systems (TECS)},
	volume={16},
	number={5s},
	pages={151},
	year={2017},
	publisher={ACM}
}
@article{wu2017squeezeseg,
	title={Squeezeseg: Convolutional neural nets with recurrent crf for real-time road-object segmentation from 3d lidar point cloud},
	author={Wu, Bichen and Wan, Alvin and Yue, Xiangyu and Keutzer, Kurt},
	journal={arXiv preprint arXiv:1710.07368},
	year={2017}
}
@article{howard2017mobilenets,
	title={Mobilenets: Efficient convolutional neural networks for mobile vision applications},
	author={Howard, Andrew G and Zhu, Menglong and Chen, Bo and Kalenichenko, Dmitry and Wang, Weijun and Weyand, Tobias and Andreetto, Marco and Adam, Hartwig},
	journal={arXiv preprint arXiv:1704.04861},
	year={2017}
}
@article{zhang2017shufflenet,
	title={Shufflenet: An extremely efficient convolutional neural network for mobile devices},
	author={Zhang, Xiangyu and Zhou, Xinyu and Lin, Mengxiao and Sun, Jian},
	journal={arXiv preprint arXiv:1707.01083},
	year={2017}
}
@inproceedings{huang2017densely,
	title={Densely connected convolutional networks},
	author={Huang, Gao and Liu, Zhuang and Weinberger, Kilian Q and van der Maaten, Laurens},
	booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
	volume={1},
	number={2},
	pages={3},
	year={2017}
}
@article{huang2017condensenet,
	title={CondenseNet: An Efficient DenseNet using Learned Group Convolutions},
	author={Huang, Gao and Liu, Shichen and van der Maaten, Laurens and Weinberger, Kilian Q},
	journal={arXiv preprint arXiv:1711.09224},
	year={2017}
}
@article{gholami2018squeezenext,
	title={SqueezeNext: Hardware-Aware Neural Network Design},
	author={Gholami, Amir and Kwon, Kiseok and Wu, Bichen and Tai, Zizheng and Yue, Xiangyu and Jin, Peter and Zhao, Sicheng and Keutzer, Kurt},
	journal={arXiv preprint arXiv:1803.10615},
	year={2018}
}
@article{huang2017multi,
	title={Multi-scale dense convolutional networks for efficient prediction},
	author={Huang, Gao and Chen, Danlu and Li, Tianhong and Wu, Felix and van der Maaten, Laurens and Weinberger, Kilian Q},
	journal={arXiv preprint arXiv:1703.09844},
	year={2017}
}
@article{motamedi2017placid,
	title={PLACID: a platform for FPGA-based accelerator creation for DCNNs},
	author={Motamedi, Mohammad and Gysel, Philipp and Ghiasi, Soheil},
	journal={ACM Transactions on Multimedia Computing, Communications, and Applications (TOMM)},
	volume={13},
	number={4},
	pages={62},
	year={2017},
	publisher={ACM}
}
@article{motamedi2016fast,
	title={Fast and Energy-Efficient CNN Inference on IoT Devices},
	author={Motamedi, Mohammad and Fong, Daniel and Ghiasi, Soheil},
	journal={arXiv preprint arXiv:1611.07151},
	year={2016}
}
